Effects of Disk Warping on the Inclination Evolution of Star-Disk-Binary Systems

Several recent studies have suggested that circumstellar disks in young stellar binaries may be driven into misalignement with their host stars due to secular gravitational interactions between the star, disk and the binary companion. The disk in such systems is twisted/warped due to the gravitational torques from the oblate central star and the external companion. We calculate the disk warp profile, taking into account of bending wave propagation and viscosity in the disk. We show that for typical protostellar disk parameters, the disk warp is small, thereby justifying the "flat-disk" approximation adopted in previous theoretical studies. However, the viscous dissipation associated with the small disk warp/twist tends to drive the disk toward alignment with the binary or the central star. We calculate the relevant timescales for the alignment. We find the alignment is effective for sufficiently cold disks with strong external torques, especially for systems with rapidly rotating stars, but is ineffective for the majority of star-disk-binary systems. Viscous warp driven alignment may be necessary to account for the observed spin-orbit alignment in multi-planet systems if these systems are accompanied by an inclined binary companion.

==> ms.tex <==
\title[Hydrodynamical Lidov-Kozai Instability]
{Lidov-Kozai Mechanism in Hydrodynamical Disks: Linear Stability Analysis}

\author[J. J. Zanazzi and Dong Lai]{J. J. Zanazzi$^{1}$\thanks{Email: jjz54@cornell.edu}, and Dong Lai$^{1}$ \\
$^{1}$Cornell Center for Astrophysics and Planetary Science, Department of Astronomy, Cornell University, Ithaca, NY 14853, USA}

\begin{abstract}
Recent SPH simulations by \cite{Martin(2014)} suggest that a
circumstellar gaseous disk may exhibit coherent
eccentricity-inclination oscillations due to the tidal forcing of an
inclined binary companion, in a manner that resembles Lidov-Kozai
oscillations in hierarchical triple systems. We carry out linear
stability analysis for the eccentricity growth of circumstellar disks
in binaries, including the effects of gas pressure and viscosity 
and secular (orbital-averaged) tidal force from the inclined
companion. We find that the growth of disk eccentricity
depends on the dimensionless ratio ($S$) between $c_s^2$ (the disk sound
speed squared) and the tidal torque acting on the disk (per unit mass)
from the companion.  For $S\ll 1$, the standard Lidov-Kozai result is
recovered for a thin disk annulus: eccentricity excitation occurs when the
mutual inclination $I$ between the disk and binary lies between $39^\circ$ and
$141^\circ$. As $S$ increases, the inclination window for eccentricity
growth generally becomes narrower. For $S\gtrsim$ a few, eccentricity
growth is suppressed for all inclination angles. Surprisingly,
we find that for $S\sim 1$ and certain disk density/pressure profiles,
eccentricity excitation can occur even when $I$ is much less than $39^\circ$.
%Our analytic results can be used to determine if a hydrodynamical
%circumstellar disk is susceptible to LK oscillations, without
%resorting to expensive SPH simulations.
\end{abstract}



%%%%%%%%%%%%%%%%%%%%%
\section{Summary and Discussion}
\label{sec:discussion}

\subsection{Summary of Key Results}
\label{sec:Summary}

Using linear theory of eccentric disturbances in hydrodynamical disks,
we have shown that circumstellar disks in binary systems may undergo
coherent eccentricity growth when the disk is significantly inclined
with respect to binary orbital plane. We consider the regime where the
disk remains approximately flat and undergoes rigid-body nodal
precession around the binary; this requires that bending waves
efficiently communicate warps in different regions of the disk within
the precession period. We find that the disk's eccentricity response to the 
secular tidal forcing from the binary companion depends crucially on the dimensionless
ratio [see Eq.~\eqref{eq:S}], 
\be
S=\left({c_s^2\over 3GMbr^2/4a^3}\right)_{r=r_{\rm out}},
\ee
where $c_2^2$ (disk sound speed squared) measures the characteristic
torque (per unit mass) associated with gas pressure, 
$3GM_br^2/a^3$ (with $M_b$ and $a$ the companion mass and semi-major
axis) measures the tidal torque from the companion. 
The eccentricty response also depends on the disk's radial extent 
($r_{\rm out}/r_{\rm in}$) and density and sound speed profiles (Eqs.xx and xx).
\begin{enumerate}
\item When $S \ll 1$, the ``standard" Lidov-Kozai effect is reproduced for a thin
disk annulus ($r_{\rm out}/r_{\rm in}\rightarrow 1$), with exponential
eccentricity growth occuring for disk inclination $I$ (with
respect to the binary orbital plane) between $39^\circ$ and $141^\circ$.
\item As $S$ increases, the inclination window for disk eccentricity growth generally 
decreases. When $S \gg 1$, eccentricity growth is completely quenched for all disk inclinations.
\item When $S \sim 1$, a ``window of instability'' is achieved for certain disk parameters,  
where coherent disk eccentricity growth is observed for inclinations $I$ outside the
standard $(39^\circ,141^\circ)$ window.
\end{enumerate}
These conclusions are qualitatively robust, shown through both analytic
calculations when the disk's radial extent is negligible (thin annulus; 
Sec.~\ref{sec:thinannulus}) and numerical eigenmode analyses when the disk
has a significant radial extent (Sec.~\ref{sec:extenddisk}).
We find that viscosity does little to quench the Lidov-Kozai instability of the disk
(Sec.~\ref{sec:viscosity}).

The different disk eccentricty responses to the secular tidal forcing 
%for different disk parameters ($S$ and density/pressure profiles)
can be understood in terms of the apsidal precession produced by gas pressure
(i.e. \citealt{Papaloizou(2002),GoodchildOgilvie(2006),TeyssandierOgilvie(2016)}).
This precession depends on the $S$ and the disk density/pressure
profiles.  Unlike the other short-range forces (such as those due to
General Relarivity and tidal interaction) in hierarchical triple
systems (e.g. Liu et al.~2015), the pressure-induced precession can be
either prograde or retrograde, depending on the disk profiles
(see Eq.~xxx; see also \citealt{TeyssandierOgilvie(2016)}).  This
gives rise to the nontrivial behavior of the disk's eccentricity
response for $S\sim 1$.

%%%%%%%%%%%%%%%
\subsection{Discussion}
%\label{sec:AddHydro}

In this paper we have focused on the linear regime of the disk
Lidov-Kozai instability, which manifests as the coherent growth of
disk eccentricity, with no change in the disk inclination (which
enters at the order $e^2$). Numerical simulations are necessary to
fully understand the nonlinear development of the disk
eccentricity-inclination oscillations (Martin et al...Fu, et al).
Nevertheless, our analytic results can be used to determine under what
conditions a hydrodynamical circumstellar disk is susceptible to
Kidov-Kozai oscillations, without resorting to full 3D numerical
simulations.

We note that the dynamical behavior of eccentric disturbances in a
hydrodynamical disk depends on the disk's equation of state and
vertical structure \citep{GoodchildOgilvie(2006),Ogilvie(2008),TeyssandierOgilvie(2016)}.
We have adopted the eccentric disk models with locally isothermal
equation of state. Using different models can change the details of
our results, but not the general conclusions summarized in Section 4.1.

The disk eccentricity excitation mechanism studied in this paper is
distinct from the mechanism that relies on eccentric Lindblad
resonance (Lubow 1991). The latter operates on the dynamical timescale
and requires that the disk be sufficiently extended relative to the
binary separation (i.e., $r_{\rm out}/a$ is sufficiently larger) so
that the resonance resides in the disk. By contrast, the disk Lidov-Kozai 
mechanism for eccentricity excitation requires an inclined binary companion, and
operates on a secular timescale [Eq.~\eqref{eq:omb}]
\begin{eqnarray}
&& t_{\rm LK}\sim \omega_b(r_{\rm out})^{-1}
= 5.7\times 10^3\,{\rm years}\left(\frac{M}{\Mb}\right)\left(\frac{a}{3 \rout}\right)^3 
\nonumber\\
&&\times\left(\frac{M}{1 M_\odot}\right)^{-1/2}\left(\frac{\rout}{100 \,\text{AU}}\right)^{3/2}.
\end{eqnarray}
For protoplanetary disks, this timescale is much less than the disk lifetime (a few Myrs).
To avoid suppression of the instability by the gas pressure, we also require
\begin{equation}
S = 0.36 \left( \frac{a}{3\,\rout}\right)^3 \left(\frac{M}{\Mb}\right)
\left( \frac{H(\rout)}{0.1 \, \rout} \right)^2 \lesssim 1.
\end{equation}
Thus, a ``weaker'' companion (large $a$ and small $M_b$) would not excite
eccentricity in a thick (large $H/R$) disk.


\section*{Acknowledgments}

This work has been supported in part by NASA grants NNX14AG94G and
NNX14AP31G, and a Simons Fellowship from the Simons Foundation.  JZ is
supported by a NASA Earth and Space Sciences Fellowship in
Astrophysics.



